Characterizing the NP-PSPACE Gap in the Satisfiability Problem for Modal Logic

There has been a great of work on characterizing the complexity of the satisfiability and validity problem for modal logics. In particular, Ladner showed that the validity problem for all logics between K, T, and S4 is {\sl PSPACE}-complete, while for S5 it is {\sl NP}-complete. We show that, in a precise sense, it is \emph{negative introspection}, the axiom $\neg K p \rimp K \neg K p$, that causes the gap. In a precise sense, if we require this axiom, then the satisfiability problem is {\sl NP}-complete; without it, it is {\sl PSPACE}-complete.

==> bghkmac.tex <==

\newenvironment{oldthm}[1]{\par\noindent{\bf Theorem #1:} \em \noindent}{\par}
\newenvironment{oldlem}[1]{\par\noindent{\bf Lemma #1:} \em \noindent}{\par}
\newenvironment{oldcor}[1]{\par\noindent{\bf Corollary #1:} \em \noindent}{\par}
\newenvironment{oldpro}[1]{\par\noindent{\bf Proposition #1:} \em \noindent}{\par}
\newcommand{\othm}[1]{\begin{oldthm}{\ref{#1}}}
\newcommand{\eothm}{\end{oldthm} \medskip}
\newcommand{\olem}[1]{\begin{oldlem}{\ref{#1}}}
\newcommand{\eolem}{\end{oldlem} \medskip}
\newcommand{\ocor}[1]{\begin{oldcor}{\ref{#1}}}
\newcommand{\eocor}{\end{oldcor} \medskip}
\newcommand{\opro}[1]{\begin{oldpro}{\ref{#1}}}
\newcommand{\eopro}{\end{oldpro} \medskip}


%general miscellanous
\newcommand{\world}{W}
\newcommand{\WN}{\W_N}
\newcommand{\Winf}{\W^*}
\newcommand{\tends}{\rightarrow}
\newcommand{\tendsto}{\tends}
\newcommand{\ninfty}{{N \rightarrow \infty}}
\newcommand{\nworldsv}[1]{{\it \#worlds}^{#1}}
\newcommand{\nworlds}{{{\it \#worlds}}_{N}^{\epsvec}}
\newcommand{\nwrldPnt}[1]{\nworlds[#1]}
\newcommand{\nworldsarg}[1]{\nworlds[#1]}
\newcommand{\binco}[2]{{{#1}\choose{#2}}}
\newcommand{\closure}[1]{{\overline{#1}}}
\newcommand{\balpha}{\bar{\alpha}}
\newcommand{\bbeta}{\bar{\beta}}
\newcommand{\bgamma}{\bar{\gamma}}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\bQ}{\overline{Q}}
%FB4: added
\newcommand{\Vector}[1]{{\langle #1 \rangle}}
%algorithms
\newcommand{\Algzeroone}{\mbox{\em Compute01}}
\newcommand{\Algcompute}{\mbox{{\em Compute-Pr}$_\infty$}}


% probabilities
\newcommand{\Prinfv}[1]{{\Pr}^{#1}_\infty}
\newcommand{\PrNv}[1]{{\Pr}^{#1}_N}
\newcommand{\Prinf}{{\Pr}_\infty}
\newcommand{\PrN}{{\Pr}_N}
\newcommand{\pN}{\PrN (\phi | \KB)}
\newcommand{\IPrinf}{{\Box\Diamond\Prinf}}
\newcommand{\PPrinf}{{\Diamond\Box\Prinf}}
\newcommand{\prNw}{{\Pr}_{N}^{\epsvec}}
\newcommand{\prNwi}{{\Pr}_{N^i}^{\epsvec^i}}
\newcommand{\priw}{{\Pr}_{\infty}}
\newcommand{\beliefprob}[1]{\Pr(#1)} %daphne1 - changed macro
\newcommand{\Prinfeps}{{{\Pr}_\infty^{\epsvec}}}
\newcommand{\PrNeps}{{{\Pr}_N^{\epsvec}}}
\newcommand{\Pinf}[2]{{\Pi_\infty^{#1}[#2]}}

% vocabularies
\newcommand{\infvocab}{\Omega}
\newcommand{\infunvocab}{\Upsilon}
\newcommand{\vocab}{\Phi}
\newcommand{\nonunaryvocab}{\vocab}
\newcommand{\unvocab}{\Psi}

% languages
\newcommand{\cL}{{\cal L}}
\newcommand{\cLne}{{\cal L}^-}
\newcommand{\finitelang}{\cL_i^d(\Phi)}
\newcommand{\fLd}{\cL_d^d(\Phi)}
\newcommand{\cLd}{\cL_{\mbox{\em \scriptsize$d$}}(\Phi)}
\newcommand{\Laeq}{{\cal L}^{\aeq}}
\newcommand{\Leq}{{\cal L}^{=}}
\newcommand{\Lunaeq}{\Laeq_1}
\newcommand{\Luneq}{\Leq_1}


%formulas
\newcommand{\KB}{{\it KB}}
 %GHK1a
\newcommand{\phieven}{\phi_{\mbox{\footnotesize\it even}}}
\newcommand{\phiodd}{\phi_{\mbox{\footnotesize\it odd}}}
\newcommand{\KBM}{\KB_{\boldM}}
 %GHK1b
\newcommand{\Pstar}{P^*}
\newcommand{\barP}{\neg P}
\newcommand{\barQ}{\neg Q}
\newcommand{\maxarity}{\rho}
\newcommand{\Init}{\mbox{\it Init\/}}
\newcommand{\Rep}{\mbox{\it Rep\/}}
\newcommand{\Acc}{\mbox{\it Acc\/}}
\newcommand{\Comp}{\mbox{\it Comp\/}}
\newcommand{\Step}{\mbox{\it Step\/}}
\newcommand{\Univ}{\mbox{\it Univ\/}}
\newcommand{\Exis}{\mbox{\it Exis\/}}
\newcommand{\Between}{\mbox{\it Between\/}}
\newcommand{\Count}{\mbox{\it count\/}}
\newcommand{\phiq}{\phi_Q}
\newcommand{\propform}{\beta}
\newcommand{\allphi}{\ast}
\newcommand{\ID}{\mbox{\it ID}}
\newcommand{\atomdesc}{{\psi_*}}
\newcommand{\rigid}{\mbox{\it rigid}}
\newcommand{\abdesc}{\widehat{D}}
\newcommand{\KBtwo}{\theta}
\newcommand{\psits}{\psi[\KBtwo,\abdesc]}
\newcommand{\psitsnohat}{\psi[\KBtwo,D]}
%BGHK
\newcommand{\KBfly}{\KB_{\mbox{\scriptsize \it fly}}}
\newcommand{\KBchirps}{\KB_{\mbox{\scriptsize \it chirps}}}
\newcommand{\KBmagpie}{\KB_{\mbox{\scriptsize \it magpie}}}
\newcommand{\KBhep}{\KB_{\mbox{\scriptsize \it hep}}}
\newcommand{\KBnixon}{\KB_{\mbox{\scriptsize \it Nixon}}}
\newcommand{\KBel}{\KB_{\mbox{\scriptsize \it likes}}}
\newcommand{\KBtax}{\KB_{\mbox{\scriptsize \it taxonomy}}}
\newcommand{\KBarm}{\KB_{\mbox{\scriptsize \it arm}}}
\newcommand{\KBlate}{\KB_{\mbox{\scriptsize \it late}}}
\newcommand{\KBp}{{\KB'}}
\newcommand{\KBflyp}{\KB_{\mbox{\scriptsize \it fly}}'}
\newcommand{\KBpp}{{\KB''}}
\newcommand{\KBdef}{\KB_{\mbox{\scriptsize \it def}}}
\newcommand{\KBdishep}{\KB_{\mbox{\scriptsize \it $\lor$hep}}}

%GHK2
\newcommand{\canKB}{\widehat{\KB}}
\newcommand{\canxi}{\widehat{\xi}}
\newcommand{\KBfo}{\KB_{\it fo}}
\newcommand{\KBconst}{\psi}
\newcommand{\KBprop}{\KBp}


%predicates
\newcommand{\quak}{\mbox{\it Quaker\/}}
\newcommand{\repub}{\mbox{\it Republican\/}}
\newcommand{\pac}{\mbox{\it Pacifist\/}}
\newcommand{\Nixon}{\mbox{\it Nixon\/}}
\newcommand{\Winner}{\mbox{\it Winner\/}}
\newcommand{\Child}{\mbox{\it Child\/}}
\newcommand{\Boy}{\mbox{\it Boy\/}}
\newcommand{\Tall}{\mbox{\it Tall\/}}
\newcommand{\Elephant}{\mbox{\it Elephant\/}}
\newcommand{\Gray}{\mbox{\it Gray\/}}
\newcommand{\Yellow}{\mbox{\it Yellow\/}}
\newcommand{\Clyde}{\mbox{\it Clyde\/}}
\newcommand{\Tweety}{\mbox{\it Tweety\/}}
\newcommand{\Opus}{\mbox{\it Opus\/}}
\newcommand{\Bird}{\mbox{\it Bird\/}}
\newcommand{\Penguin}{{\it Penguin\/}}
\newcommand{\Fish}{\mbox{\it Fish\/}}
\newcommand{\Fly}{\mbox{\it Fly\/}}
\newcommand{\Warmblooded}{\mbox{\it Warm-blooded\/}}
\newcommand{\White}{\mbox{\it White\/}}
\newcommand{\Red}{\mbox{\it Red\/}}
\newcommand{\Winged}{\mbox{\it Winged\/}}
\newcommand{\Giraffe}{\mbox{\it Giraffe\/}}
\newcommand{\Visible}{\mbox{\it Easy-to-see\/}}
\newcommand{\Bat}{\mbox{\it Bat\/}}
\newcommand{\Blue}{\mbox{\it Blue\/}}
\newcommand{\Fever}{\mbox{\it Fever\/}}
\newcommand{\Jaun}{\mbox{\it Jaun\/}}
\newcommand{\Hep}{\mbox{\it Hep\/}}
\newcommand{\Eric}{\mbox{\it Eric\/}}
\newcommand{\Alice}{\mbox{\it Alice\/}}
\newcommand{\Tom}{\mbox{\it Tom\/}}
\newcommand{\Lottery}{\mbox{\it Lottery\/}}
\newcommand{\Zookeeper}{\mbox{\it Zookeeper\/}}
\newcommand{\Fred}{\mbox{\it Fred\/}}
\newcommand{\Likes}{\mbox{\it Likes\/}}
\newcommand{\Day}{\mbox{\it Day\/}}
\newcommand{\Nextday}{\mbox{\it Next-day\/}}
\newcommand{\Sleepslate}{\mbox{\it To-bed-late\/}}
\newcommand{\Riseslate}{\mbox{\it Rises-late\/}}
\newcommand{\TS}{\mbox{\it TS\/}}
\newcommand{\EEJ}{\mbox{\it EEJ\/}}
\newcommand{\FC}{\mbox{\it FC\/}}
\newcommand{\Dodo}{\mbox{\it Dodo\/}}
\newcommand{\Ab}{\mbox{\it Ab\/}}
\newcommand{\Chirps}{\mbox{\it Chirps\/}}
\newcommand{\Swims}{\mbox{\it Swims\/}}
\newcommand{\Magpie}{\mbox{\it Magpie\/}}
\newcommand{\Moody}{\mbox{\it Moody\/}}
\newcommand{\SomeMorning}{\mbox{\it Tomorrow\/}}
\newcommand{\Animal}{\mbox{\it Animal\/}}
\newcommand{\Sparrow}{\mbox{\it Sparrow\/}}
\newcommand{\Turtle}{\mbox{\it Turtle\/}}
\newcommand{\Older}{\mbox{\it Over60\/}}
\newcommand{\Patient}{\mbox{\it Patient\/}}
\newcommand{\Black}{\mbox{\it Black\/}}
\newcommand{\Ray}{\mbox{\it Ray\/}}
\newcommand{\Reiter}{\mbox{\it Reiter\/}}
\newcommand{\Drew}{\mbox{\it Drew\/}}
\newcommand{\McDermott}{\mbox{\it McDermott\/}}
\newcommand{\Emu}{\mbox{\it Emu\/}}
\newcommand{\Canary}{\mbox{\it Canary\/}}
\newcommand{\BlueCanary}{\mbox{\it BlueCanary\/}}
\newcommand{\FlyingBird}{\mbox{\it FlyingBird\/}}
\newcommand{\UL}{\mbox{\it LeftUsable\/}}
\newcommand{\UR}{\mbox{\it RightUsable\/}}
\newcommand{\BL}{\mbox{\it LeftBroken\/}}
\newcommand{\BR}{\mbox{\it RightBroken\/}}
\newcommand{\Ticket}{\mbox{\it Ticket\/}}
\newcommand{\BlueEyed}{{\mbox{\it BlueEyed\/}}}
\newcommand{\Jaundice}{{\it Jaundice\/}}
\newcommand{\Hepatitis}{{\it Hepatitis\/}}
\newcommand{\HeartDisease}{{\mbox{\it Heart-disease\/}}}
\newcommand{\bJ}{{\overline{J}\,}}
\newcommand{\bH}{{\overline{H}\,}}
\newcommand{\bB}{{\overline{B}\,}}
\newcommand{\Prem}{{\mbox{\it Child\/}}}
\newcommand{\David}{{\mbox{\it David\/}}}
\newcommand{\Son}{{\mbox{\it Son\/}}}	% changed


%miscellaneous  GHK1a+b
\newcommand{\ceslim}{Ces\`{a}ro limit}
\newcommand{\Sigmad}{\Sigma^d_i}
\newcommand{\Liogonkii}{Liogon'ki\u\i}
\newcommand{\Vstar}{{\modfrag_*}}
\newcommand{\moddesc}{\psi \land \modfrag}
\newcommand{\sumact}{\Degr_2}
\newcommand{\degree}{\Degr_1}
\newcommand{\Active}{\alpha}
\newcommand{\ActiveAtoms}{\boldA}
\newcommand{\named}{n}
\newcommand{\aactive}{a}
\newcommand{\degr}{\delta}
\newcommand{\chsize}{f}
\newcommand{\chconst}{g}
\newcommand{\Chconst}{G}
\newcommand{\Degr}{\Delta}
\newcommand{\frags}{\M}
\newcommand{\const}{H}
\newcommand{\modfrag}{\V}
\newcommand{\AD}{\A}
\newcommand{\Named}{\nu}
\newcommand{\bit}{b}
\newcommand{\guess}{\gamma}
\newcommand{\bxor}[1]{\dot{\bor}}
\newcommand{\weight}{\omega}
%\newcommand{\arity}{r}
\newcommand{\arity}{{\it arity}}
\newcommand{\assigned}{\leftarrow}
\newcommand{\snum}[2]{{{#1} \brace {#2}}}


%proportions & approximate equality
\newcommand{\eps}{\tau}
\newcommand{\vareps}{\varepsilon}
\newcommand{\varepsvec}{{\vec{\vareps}}}
\newcommand{\xtuple}{\vec{x}}
\newcommand{\ctuple}{{\vec{c}\,}}
\newcommand{\uvec}{{\!{\vec{\,u}}}}
\newcommand{\ucom}{u}
%FB4 I don't know why you set pvec, pcom to be u! But I needed a pvec,
%so I changed it. Please beware if using this for files other than
%BGHK!
%\newcommand{\pvec}{{\!{\vec{\,u}}}}
\newcommand{\pvec}{{\!{\vec{\,p}}}}
%\newcommand{\pcom}{u}
\newcommand{\pcom}{p}
\newcommand{\vvec}{\vec{v}}
\newcommand{\wvec}{\vec{w}}
\newcommand{\xvec}{\vec{x}}
\newcommand{\yvec}{\vec{y}}
\newcommand{\zvec}{\vec{z}}
\newcommand{\zerovec}{\vec{0}}

\newcommand{\epscom}{\eps}
\newcommand{\epsvec}{{\vec{\eps}\/}}
\newcommand{\prop}[2]{{||{#1}||_{{#2}}}}
\newcommand{\aeq}{\approx} %``Approximate'' connectives
\newcommand{\app}{\approx}
\newcommand{\alt}{\prec}
\newcommand{\aleq}{\preceq}
\newcommand{\agt}{\succ}
\newcommand{\ageq}{\succeq}
\newcommand{\altne}{\prec}
\newcommand{\naeq}{\not\approx}
\newcommand{\cprop}[3]{{\|{#1}|{#2}\|_{{#3}}}}
\newcommand{\Bigcprop}[3]{{\Bigl\|{#1}\Bigm|{#2}\Bigr\|_{{#3}}}}


%miscellaneous BGHK
\newcommand{\reals}{\IR}
\newcommand{\qsep}{\,}
\newcommand{\perm}{\pi}
\newcommand{\val}{V}
\newcommand{\rwent}{\mbox{$\;|\!\!\!\sim$}_{\mbox{\scriptsize \it rw}}\;}
\newcommand{\notrwent}{\mbox{$\;|\!\!\!\not\sim$}_{\mbox{\scriptsize\it rw}}\;}
\newcommand{\dempster}{\delta}
\newcommand{\dentails}{{\;|\!\!\!\sim\;}}
\newcommand{\notdentails}{{\;|\!\!\!\not\sim\;}}
\newcommand{\dentailssub}[1]{\dentails\hspace{-0.4em}_{
          \mbox{\scriptsize{\it #1}}}\;}
\newcommand{\notdentailssub}[1]{\notdentails\hspace{-0.4em}_{
          \mbox{\scriptsize{\it #1}}}\;}
\newcommand{\default}{\rightarrow}

%miscellaneous GHK2
\newcommand{\vecof}[1]{{\pi({#1})}}
\newcommand{\PIN}[2]{{\Pi_N^{#1}[#2]}}
\newcommand{\SS}[2]{{S^{#1}[#2]}}
\newcommand{\SSc}[2]{{S^{#1}[#2]}}
\newcommand{\SSzero}[1]{\SS{\zerovec}{#1}}
\newcommand{\SSczero}[1]{\SSc{\zerovec}{#1}}
\newcommand{\SSpos}[1]{\SS{\leq \zerovec}{#1}}
\newcommand{\Sol}{{\it Sol}}
\newcommand{\poscon}{\gamma}
\newcommand{\constraints}{\Gamma}
\newcommand{\constpos}{\constraints^{\leq}}
%\newcommand{\vareps}{\varepsilon}
\newcommand{\propspace}{\Delta^K}
\newcommand{\mept}{\vvec}
\newcommand{\mecoord}{v}
\newcommand{\mepts}{{\Q}}
\newcommand{\OS}{{\cal O}}
\renewcommand{\S}{{\cal S}}
\newcommand{\meval}{{\rho}}
\newcommand{\meptmin}{{\uvec^{\ast}_{\mbox{\scriptsize min}}}}
\newcommand{\sizeof}[1]{{\sigma(#1)}}
\newcommand{\mesize}{{\sigma^{\ast}}}
\renewcommand{\pf}{\alpha}
\newcommand{\ps}{\beta}
\newcommand{\Atoms}{\AD}
\newcommand{\limNstar}{{\lim_{N \rightarrow \infty}}^{\!\!\!*}\:}
\newcommand{\probf}[2]{F_{[#1|#2]}}
\newcommand{\probfun}[1]{F_{[#1]}}
\newcommand{\Prmu}[1]{{\mu}_{#1}}
\newcommand{\foversion}[1]{\xi_{#1}}
\newcommand{\fly}{\mbox{\it fly\/}}
\newcommand{\bird}{\mbox{\it bird\/}}
\newcommand{\yellow}{\mbox{\it yellow\/}}
\newcommand{\propconsts}{\Lambda}
\newcommand{\alldiff}{\chi^{\neq}}
\newcommand{\unaryD}{D^1}
\newcommand{\nonunD}{D^{> 1}}
\newcommand{\eqD}{D^{=}}



==> spage.tex <==

\setlength{\evensidemargin}{0in}
\setlength{\oddsidemargin}{0in}
\setlength{\textwidth}{6.25in}
\setlength{\textheight}{8.5in}
\setlength{\topmargin}{0in}
\setlength{\headheight}{0in}
\setlength{\headsep}{0in}
%\setlength{\itemsep}{-\parsep}
\setlength{\itemsep}{0pt}
\renewcommand{\topfraction}{.9}
\renewcommand{\textfraction}{.1}
\setlength{\parskip}{\smallskipamount}


